The Impact of Observing Strategy on Cosmological Constraints with LSST

The generation-defining Vera C. Rubin Observatory will make state-of-the-art measurements of both the static and transient universe through its Legacy Survey for Space and Time (LSST). With such capabilities, it is immensely challenging to optimize the LSST observing strategy across the survey's wide range of science drivers. Many aspects of the LSST observing strategy relevant to the LSST Dark Energy Science Collaboration, such as survey footprint definition, single visit exposure time and the cadence of repeat visits in different filters, are yet to be finalized. Here, we present metrics used to assess the impact of observing strategy on the cosmological probes considered most sensitive to survey design; these are large-scale structure, weak lensing, type Ia supernovae, kilonovae and strong lens systems (as well as photometric redshifts, which enable many of these probes). We evaluate these metrics for over 100 different simulated potential survey designs. Our results show that multiple observing strategy decisions can profoundly impact cosmological constraints with LSST; these include adjusting the survey footprint, ensuring repeat nightly visits are taken in different filters and enforcing regular cadence. We provide public code for our metrics, which makes them readily available for evaluating further modifications to the survey design. We conclude with a set of recommendations and highlight observing strategy factors that require further research.

==> The Impact of Observing Strategy on Cosmology with LSST/author_acknowledgements.tex <==
%%%% AUTOMATICALLY GENERATED DO NOT EDIT %%%%
TA acknowledges support from Proyecto Fondecyt N 1190335 and the ANID-Millennium Science Initiative Program – ICN12\_009 awarded to the Millennium Institute of Astrophysics MAS. HAw also acknowledges support by the Rutgers Discovery Informatics Institute (RDI2) Fellowship of Excellence in Computational and Data Science, Rutgers University \& Bevier Dissertation Completion Fellowship, Leinweber Postdoctoral Research Fellowship, and DOE grant DE-SC009193. HAw also thanks the LSSTC Data Science Fellowship Program, which is funded by LSSTC, NSF Cybertraining Grant \#1829740, the Brinson Foundation, and the Moore Foundation, as participation in the program has benefited this work.  This material is based upon work supported by the U.S. Department of Energy, Office of Science, Office of High Energy Physics Cosmic Frontier Research pro- gram under Award Numbers DE-SC0011636 and DE- SC0010008, which supported EG and HAw.   SGG acknowledges support from the University of Rochester and the DOE Office of High Energy Physics under grant number DE-SC0008475. 

        
                
                
        
        
                
                        
                                
SH and SHS thank the European Research Council (ERC) for support under the European Union’s Horizon 2020 research and innovation programme (LENSNOVA: grant agreement No. 771776)

                                
                        
                
         This material is based upon work supported by the U.S. Department of Energy, Office of Science, Office of High Energy Physics Cosmic Frontier Research program under Award Numbers DE-SC0011636, which supported SWJ. AGKs work is supported by the U.S. Department of Energy, Office of Science, Office of High Energy Physics, under contract No. DE-AC02-05CH11231. ML acknowledges support from the South African Radio Astronomy Observatory and the National Research Foundation (NRF) towards this research. Opinions expressed and conclusions arrived at, are those of the authors and are not necessarily to be attributed to the NRF. RM and H. Almoubayyed are supported by the Department of Energy grant DE-SC0010118. This document was prepared by DESC using the resources of the Fermi National Accelerator Laboratory (Fermilab), a U.S. Department of Energy, Office of Science, HEP User Facility. Fermilab is managed by Fermi Research Alliance, LLC (FRA), acting under Contract No. DE-AC02-07CH11359 CS, RB and HVP's work was partially supported the research environment grant “Gravitational Radiation and Elec- tromagnetic Astrophysical Transients (GREAT)” funded by the Swedish Research Council (VR) under Dnr 2016- 06012 and the research project grant ‘Understanding the Dynamic Universe’ funded by the Knut and Alice Wallenberg Foundation under Dnr KAW 2018.0067. TP acknowledges the financial support from the Slovenian Research Agency (grants I0-0033, P1-0031, J1-8136 and Z1-1853). SHS thanks the Max Planck Society for support through the Max Planck Research Group.

                                
                        
                
         %%%% AUTOMATICALLY GENERATED DO NOT EDIT %%%%


==> The Impact of Observing Strategy on Cosmology with LSST/author_contributions.tex <==
%%%% AUTOMATICALLY GENERATED DO NOT EDIT %%%%
\noindent Author contributions are listed below.\\ 
\noindent \textbf{HAl:} Developed WL systematics metric, contributed MAF metric for 3x2pt Figure of Merit. Analysis and interpretation for weak lensing metric results. Writing and discussion for sections 4 and 6. \\
\textbf{TA:} Helped develop time delay lensed quasar metric, run metrics, analysis and discussion of Section 5.2.\\
\textbf{HAw:} Provided technical assistance with simulations. Developed MAF metrics for the extragalactic footprint and the number of galaxies. Provided numbers for basic static metrics (e.g depth statistics) and those for LSS. Helped with discussions, and writing sections 3 and 4.\\
\textbf{RB:} Contributed to software and metric development\\
\textbf{TB:} Contributed to long time-scale microlensing efficiency understanding\\
\textbf{EG:} Conceptualization, discussion, and writing in sections 3 and 4.  Edited sections 1-4 and 7.  \\
\textbf{SGG:} Section 5.1.3, metric for SNe PV\\
\textbf{PG:} Section 5.1: discussion, oversight and writing. Developed a set of supernovae metrics implemented in MAF. Processed all observing strategies. Developed real-time display (\url{https://me.lsst.eu/gris/OS_Videos/}) to visualize the progress of observing strategies on a daily basis to study cadence/gap effects. Implementation of the lensed SNe Ia by galaxies metric in MAF and processing of observing strategies (section 5.2.1).\\
\textbf{IH:} Section 5.1:discussion. Writing (review and editing) of Sections 1,2 and 5.\\
\textbf{SH:}  Section 5.2.1:metric, Section 5.2:validation, analysis, writing, editing, \\
\textbf{SWJ:} Conceptualization and development of observing strategies related to SN Ia (section 5.1) and rolling cadences. Editing of sections 1 and 2.\\
\textbf{RLJ:} Created simulations, technical assistance with simulations and metric interpretation. Worked with various groups to develop metrics and analysis.\\
\textbf{AGK:} Section 5.1.3, writing/metric-creation\\
\textbf{ML:} Conceptualization,  software, validation, formal analysis, investigation, data curation, writing - original draft, writing - review and editing, visualization, supervision\\
\textbf{RM:} Discussion and writing in sections 3 and 4\\
\textbf{PM:} Section 5.2 (designed and implemented metrics, wrote text)\\
\textbf{MM:} Microlensing discussion and writing in introduction\\
\textbf{EHN:} Improved seeing input to opsim simulations (section 2.5, 6.7), general descussions and recommendations\\
\textbf{HP:} Section 5.3: conceptualization, validation, writing - review, supervision, funding acquisition\\
\textbf{TP:} Metric development and writing of subsection 5.2.2\\
\textbf{NR:} Section 5.1: discussion and writing. Developed a set of metrics to evaluate the expected quality on the SN light curves, on the DDF and WFD surveys. Built a pipeline to evaluate the pre-white paper, white-paper and fbs1.3 - fbs1.7 cadences. \\
\textbf{DR:} Developed deterministic scheduler (alt sched) as a conceptual alternative to OpSim for comparison purposes\\
\textbf{DS:} Conceptualization,  writing - original draft, writing - review \& editing, visualization, supervision\\
\textbf{CNS:} Software, metrics, validation, analysis and writing of Section 5.3.\\
\textbf{CS:} Developed deterministic scheduler (alt sched) as a conceptual alternative to OpSim for comparison purposes\\
\textbf{SHS:} Coordinated strong lensing group; writing, validation, analysis and editing of Section 5.2.\\
\textbf{PY:} Created survey simulations. Section 2 writing. Helped with development of MAF metrics for Section 3, 5.\\
%%%% AUTOMATICALLY GENERATED DO NOT EDIT %%%%


==> The Impact of Observing Strategy on Cosmology with LSST/authors.tex <==
%%%% AUTOMATICALLY GENERATED DO NOT EDIT %%%%
\author{Michelle Lochner} 
\affiliation{Department of Physics and Astronomy, University of the Western Cape, Bellville, Cape Town, 7535, South Africa} 
\affiliation{South African Radio Astronomy Observatory (SARAO), The Park, Park Road, Pinelands, Cape Town 7405, South Africa} 

\author{Dan Scolnic} 
\affiliation{Department of Physics, Duke University, 120 Science Drive, Durham, NC, 27708, USA} 

\author{Husni Almoubayyed} 
\affiliation{McWilliams Center for Cosmology, Department of Physics, Carnegie Mellon University, Pittsburgh, PA 15213, USA} 

\author{Timo Anguita} 
\affiliation{Departamento de Ciencias Fisicas, Universidad Andres Bello, Fernandez Concha 700, Las Condes, Santiago, Chile} 
\affiliation{Millennium Institute of Astrophysics, Nuncio Monsenor Sotero Sanz 100, Of. 104, Providencia, Santiago, Chile } 

\author{Humna Awan} 
\affiliation{Leinweber Center for Theoretical Physics, Department of Physics, University of Michigan, Ann Arbor, MI 48109, USA} 
\affiliation{Department of Physics and Astronomy, Rutgers, the State University, Piscataway, NJ 08854, USA} 

\author{Eric Gawiser} 
\affiliation{Department of Physics and Astronomy, Rutgers, the State University, Piscataway, NJ 08854, USA} 

\author{Satya Gontcho A Gontcho} 
\affiliation{Department of Physics \& Astronomy, University of Rochester, 500 Wilson Blvd., Rochester, NY 14627} 

\author{Philippe Gris} 
\affiliation{Laboratoire de Physique de Clermont,IN2P3/CNRS, Universit\'e Clermont Auvergne, F-63000 Clermont-Ferrand, France} 

\author{Simon Huber} 
\affiliation{Max-Planck-Institut f{\"u}r Astrophysik, Karl-Schwarzschild-Str.~1, 85748 Garching, Germany} 
\affiliation{Physik-Department, Technische Universit\"at M\"unchen, James-Franck-Stra\ss{}e~1, 85748 Garching, Germany} 

\author{Saurabh W. Jha} 
\affiliation{Department of Physics and Astronomy, Rutgers, the State University, Piscataway, NJ 08854, USA} 

\author{R. Lynne  Jones} 
\affiliation{Department of Astronomy, University of Washington, Seattle, WA  98195, USA} 
\affiliation{DiRAC Institute, University of Washington, Seattle, WA  98195, USA} 

\author{Alex G. Kim} 
\affiliation{Lawrence Berkeley National Laboratory, 1 Cyclotron Rd., Berkeley, CA, 94720, USA} 

\author{Rachel Mandelbaum} 
\affiliation{McWilliams Center for Cosmology, Department of Physics, Carnegie Mellon University, Pittsburgh, PA 15213, USA} 

\author{Phil Marshall} 
\affiliation{Kavli Institute for Particle Astrophysics and Cosmology,
P.O. Box 20450, MS29,
Stanford,
CA 94309,
U.S.A.} 

\author{Tanja Petrushevska} 
\affiliation{Centre for Astrophysics and Cosmology, University of Nova Gorica, Vipavska 11c, 5270 Ajdov\v{s}\u{c}ina, Slovenia} 

\author{Nicolas Regnault} 
\affiliation{Laboratoire de Physique Nucleaire et de Hautes-Energies, Barre 12-22 1er etage, 4 place Jussieu, 75005 Paris, France} 

\author{Christian N. Setzer} 
\affiliation{The Oskar Klein Centre for Cosmoparticle Physics, Department of Physics, Stockholm University, AlbaNova, Stockholm, SE-106 91, Sweden} 

\author{Sherry H. Suyu} 
\affiliation{Max-Planck-Institut f{\"u}r Astrophysik, Karl-Schwarzschild-Str.~1, 85748 Garching, Germany} 
\affiliation{Physik-Department, Technische Universit\"at M\"unchen, James-Franck-Stra\ss{}e~1, 85748 Garching, Germany} 
\affiliation{Academia Sinica Institute of Astronomy and Astrophysics (ASIAA), 11F of ASMAB, No.1, Section 4, Roosevelt Road, Taipei 10617, Taiwan} 

\author{Peter Yoachim} 
\affiliation{Department of Astronomy, University of Washington, Seattle, WA  98195, USA} 

\author{Rahul  Biswas} 
\affiliation{The Oskar Klein Centre for Cosmoparticle Physics, Department of Physics, Stockholm University, AlbaNova, Stockholm, SE-106 91, Sweden} 

\author{Tristan Blaineau} 
\affiliation{Universit\'e Paris-Saclay, CNRS/IN2P3, IJCLab, 91405 Orsay, France} 

\author{Isobel Hook} 
\affiliation{Department of Physics, Lancaster University, Lancaster, Lancs LA1 4YB, U.K.} 

\author{Marc Moniez} 
\affiliation{Universit\'e Paris-Saclay, CNRS/IN2P3, IJCLab, 91405 Orsay, France} 

\author{Eric Neilsen} 
\affiliation{Fermi National Accelerator Laboratory, P.O. Box 500, Batavia, IL 60510, USA} 

\author{Hiranya Peiris} 
\affiliation{The Oskar Klein Centre for Cosmoparticle Physics, Department of Physics, Stockholm University, AlbaNova, Stockholm, SE-106 91, Sweden} 
\affiliation{Department of Physics \& Astronomy, University College London, Gower Street, London WC1E 6BT, UK} 

\author{Daniel Rothchild} 
\affiliation{Department of Electrical Engineering and Computer Sciences, UC Berkeley, 253 Cory Hall, Berkeley, CA 94720-1770} 

\author{Christopher Stubbs} 
\affiliation{Department of Physics, Harvard University, 17 Oxford St, Cambridge MA 02138} 
\affiliation{Department of Astronomy, Harvard University, 60 Garden St, Cambridge MA 02138} 

\author{the LSST Dark Energy Science Collaboration}
%%%% AUTOMATICALLY GENERATED DO NOT EDIT %%%%


==> The Impact of Observing Strategy on Cosmology with LSST/desc_acknowledgements.tex <==
The DESC acknowledges ongoing support from the Institut National de 
Physique Nucl\'eaire et de Physique des Particules in France; the 
Science \& Technology Facilities Council in the United Kingdom; and the
Department of Energy, the National Science Foundation, and the LSST 
Corporation in the United States.  DESC uses resources of the IN2P3 
Computing Center (CC-IN2P3--Lyon/Villeurbanne - France) funded by the 
Centre National de la Recherche Scientifique; the National Energy 
Research Scientific Computing Center, a DOE Office of Science User 
Facility supported by the Office of Science of the U.S.\ Department of
Energy under Contract No.\ DE-AC02-05CH11231; STFC DiRAC HPC Facilities, 
funded by UK BIS National E-infrastructure capital grants; and the UK 
particle physics grid, supported by the GridPP Collaboration.  This 
work was performed in part under DOE Contract DE-AC02-76SF00515. This paper has undergone internal review in the LSST Dark Energy Science Collaboration. The authors thank the internal reviewers, who were Ariel Goobar, Joshua Meyers and Samuel Schmidt. The authors also thank Jean-Charles Cuillande and Christopher Frohmaier for providing the footprint maps for Euclid and 4MOST respectively.
